Evaluating Text-to-Image and Text-to-Video Synthesis with a Conditional Fr\'{e}chet Distance

Evaluating text-to-image and text-to-video models is challenging due to a fundamental disconnect: established metrics fail to jointly measure visual quality and semantic alignment with text, leading to a poor correlation with human judgments. To address this critical issue, we propose cFreD, a general metric based on a Conditional Fr\'echet Distance that unifies the assessment of visual fidelity and text-prompt consistency into a single score. Existing metrics such as Fr\'echet Inception Distance (FID) capture image quality but ignore text conditioning while alignment scores such as CLIPScore are insensitive to visual quality. Furthermore, learned preference models require constant retraining and are unlikely to generalize to novel architectures or out-of-distribution prompts. Through extensive experiments across multiple recently proposed text-to-image models and diverse prompt datasets, cFreD exhibits a higher correlation with human judgments compared to statistical metrics , including metrics trained with human preferences. Our findings validate cFreD as a robust, future-proof metric for the systematic evaluation of text conditioned models, standardizing benchmarking in this rapidly evolving field. We release our evaluation toolkit and benchmark.

==> Table/HPDv2_train.tex <==
\begin{table*}[t]
\centering
%\small
\renewcommand\tabcolsep{3pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc|cccccc}
\toprule
\multirow{3}{*}{Models \& Metric} & \multicolumn{12}{c}{Automatic Metric }                              & \multicolumn{6}{|c}{Human Preference Trained Model}                                   \\ \cmidrule(l){2-11} \cmidrule(l){12-19} 
& \multicolumn{2}{c}{Human Eval.$\uparrow$} & \multicolumn{2}{c}{FID$\downarrow$} & \multicolumn{2}{c}{$\text{FD}_{\text{\tiny{DINOv2}}}\downarrow$} & \multicolumn{2}{c}{CLIP$\uparrow$} &  \multicolumn{2}{c}{CMMD$\downarrow$} & \multicolumn{2}{c}{cFID$\downarrow$} &\multicolumn{2}{|c}{ Aesthetic Score$\uparrow$} &\multicolumn{2}{c}{ImageReward$\uparrow$} & \multicolumn{2}{c}{MPS$\uparrow$} 
\\ \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9} \cmidrule(l){10-11} \cmidrule(l){12-13} \cmidrule(l){14-15} \cmidrule(l){16-17} \cmidrule(l){18-19} 
            & Rank    & Rate     & Rank   & Score    & Rank & Score       & Rank    & Score    & Rank  & Score   & Rank  & Score   & Rank  & Score   & Rank   & Score   & Rank & Score  \\ \midrule
CogView2    & 4       & 33.37\%   & 4     & 20.62    & 4      & 21.25     & 1      & 16.45     & 4     & 38.10   &       &         & 4     &  4.53   & 4      & -1.1949 & 4    & 7.93       \\
DALLE 2     & 2       & 71.32\%   & 2     & 2.78     & 2      & 2.10      & 4      & 15.71     & 2     & 2.14    &       &         & 2     &  5.63   & 3      & 0.1815  & 2    & 13.02             \\
SD v1.4     & 1       & 74.69\%   & 1     & 2.22     & 1      & 1.83      & 3      & 15.85     & 1     & 1.14    &       &         & 1     &  5.70   & 1      & 0.4099  & 1    & 13.42         \\
SD v2.0     & 3       & 70.62\%   & 3     & 5.01     & 3      & 3.89      & 2      & 16.21     & 3     & 4.17    &       &         & 3     &  5.45   & 2      & 0.3832  & 3    & 12.95            
 \\\midrule
correlation to Human Eval.  & \multicolumn{2}{c}{-}  &  \multicolumn{2}{c}{0.99} & \multicolumn{2}{c}{1.00} & \multicolumn{2}{c}{0.64}  &  \multicolumn{2}{c}{1.00} & \multicolumn{2}{c}{0.} \vline & \multicolumn{2}{c}{0.99}                & \multicolumn{2}{c}{0.99}  & \multicolumn{2}{c}{1.00}        \\ %\midrule
 \bottomrule
\end{tabular}
}
\caption{Text-to-image model ranking by automatic metrics (FID, $\text{FD}_{\text{\tiny{DINOv2}}}$, CLIP score, CMMD, and cFID) and models that were trained with human preference (Aesthetic Score, ImageReward, and MPS) on HPDv2 train set.}
\label{tab:HPSv2_train_rank}
\end{table*}




==> Table/Human_Preference_Trained_Metrics.tex <==
\begin{table}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}

\scalebox{0.52}{
\begin{tabular}{lccccccccccc}
\toprule
\multicolumn{11}{c}{\textbf{(a) Text-to-Image Evaluation}} \\
\midrule
\multirow{2}{*}{\textbf{Dataset}}&
\multicolumn{2}{c}{\textbf{Aesthetic}}& 
\multicolumn{2}{c}{\textbf{ImageReward}} & 
\multicolumn{2}{c}{\textbf{HPSv2}} &   
\multicolumn{2}{c}{\textbf{MPS}} &  
\multicolumn{2}{c}{\textbf{cFreD}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
   & $\rho^2$ & Rank Acc. & $\rho^2$ & Rank Acc. & $\rho^2$ & Rank Acc. & $\rho^2$ & Rank Acc. & $\rho^2$ & Rank Acc. \\
\midrule
\textbf{HPDv2~\cite{wu2023human}}      & 0.83  & 82.2 & 0.71  & 84.4 &  0.90   & 88.9   &  0.86 & 86.7 & \textbf{0.97} & \textbf{91.1} \\
\textbf{Gen-AI Bench~\cite{lin2024evaluating}} &  0.55 & 73.3 & 0.89 & 86.7 & 0.79 & 87.7 & 0.45 & 73.3 & \textbf{0.68} & \textbf{86.7} \\
\bottomrule
\end{tabular}
}

\vspace{0.5em}

\setlength{\tabcolsep}{6pt}

\scalebox{0.7}{
\begin{tabular}{lcccccc}
\toprule
\multicolumn{7}{c}{\textbf{(b) Text-to-Video Evaluation}} \\
\midrule
\multirow{2}{*}{\textbf{Dataset}}&
\multicolumn{2}{c}{\textbf{VideoScore 1.1}}& 
\multicolumn{2}{c}{\textbf{VisionReward}} & 
\multicolumn{2}{c}{\textbf{cFreD}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
   & $\rho^2$ & Rank Acc. & $\rho^2$ & Rank Acc. & $\rho^2$ & Rank Acc. \\
\midrule
\textbf{T2VQA-DB~\cite{kou2024subjective}} & 0.02 & 55.6 & 0.01 & 46.67 & \textbf{0.86} & \textbf{91.1} \\
\textbf{EvalCrafter~\cite{liu2024evalcrafter}} & \textbf{0.91} & 20.0 & 0.27 & 60.0 & 0.90 & \textbf{100.0} \\
\bottomrule
\end{tabular}
}

\caption{Comparison of \metric (cFreD) with metrics trained using human preference across (a) text-to-image and (b) text-to-video evaluation settings. We report squared Spearman correlation ($\rho^2$) and rank accuracy (\%) with human preference. Best results are shown in \textbf{bold}.}
\label{tab:human_preference_trained_metrics}
\end{table}

==> Table/macro_acc.tex <==
\begin{table}[ht]
\centering
\small
\setlength\tabcolsep{1.5pt}
%\renewcommand{\arraystretch}{1.1}
    \begin{tabular}{c l c}
        \toprule
        & &\textbf{Macro-Accuracy (\%)} $\uparrow$ \\   
        \midrule
        \multirow{5}{*}{\shortstack{Automatic \\ Metric}} & FID & 86.7 \\
        & $\text{FD}_{\text{\tiny{DINOv2}}}$ & 86.7 \\
        & CLIPScore  & 15.6 \\
        & CMMD  & 80.0 \\
        & cFID  & \textbf{95.6} \\
        \midrule
        \multirow{4}{*}{\shortstack{Human \\ Preference \\ Trained}}
        & Aesthetic Score &  82.2\\
        & ImageReward & 84.4\\
        & HPS v2 & 88.9 \\
        & MPS &  86.7 \\
        \bottomrule
    \end{tabular}
    \caption{Macro-Accuracy on test sets of HPD v2. }
    \label{tab:macro_acc}
\end{table}
